Improving Weakly Supervised Visual Grounding by Contrastive Knowledge Distillation

Weakly supervised phrase grounding aims at learning region-phrase correspondences using only image-sentence pairs. A major challenge thus lies in the missing links between image regions and sentence phrases during training. To address this challenge, we leverage a generic object detector at training time, and propose a contrastive learning framework that accounts for both region-phrase and image-sentence matching. Our core innovation is the learning of a region-phrase score function, based on which an image-sentence score function is further constructed. Importantly, our region-phrase score function is learned by distilling from soft matching scores between the detected object names and candidate phrases within an image-sentence pair, while the image-sentence score function is supervised by ground-truth image-sentence pairs. The design of such score functions removes the need of object detection at test time, thereby significantly reducing the inference cost. Without bells and whistles, our approach achieves state-of-the-art results on visual phrase grounding, surpassing previous methods that require expensive object detectors at test time.

==> tables/cvpr-flickr30k-per-category-accuracy.tex <==
\renewcommand{\arraystretch}{0.7}
\begin{table*}[th!]
  \small
  \centering
  \resizebox{0.9\columnwidth}{!}{
  \begin{tabular}{lcccccccc}
    \toprule
   \parbox{3cm}{Method} &
   people & clothing & body parts & animals & vehicles & instruments & scene & other\\ \midrule
%   GroundeR & 44.32 & 9.02 & 0.96 & 46.91 & 46.00 & 19.14 & 28.23 & 16.98 \\
%   UTG (YOLOv2 CC) & 58.37 & 14.87 & 2.29 & 68.91 & 55.00 & 22.22 & 24.87 & 20.77 \\
%   KAC (VGG16 CC) & 58.42 & 7.63 & 2.97 & 77.80 & 69.00 & 20.37 & 43.53 & 17.05 \\
%   WPT (IRV2 CC+IRV2 OI+WRN18 PL) & 66.27 & 37.55 & 20.65 & 84.75 & 80.00 & 47.53 & 38.91 & 34.41 \\
%   \midrule

   NCE & 64.12 & 37.57 & 9.75 & 77.49 &  72.70 & 54.90 & 34.05 & 34.81 \\
   NCE+Distill & 66.20 & 40.74 & 15.77 & 76.89 & 75.21 & 60.13 & 37.15 & 35.63 \\
%   NCE & 60.09 & 54.52 & 22.20 & 60.76 &  57.38 & 23.53 & 51.58 & 38.40 \\
%   NCE+Distillation (IRV2 OI) & 61.48 & 56.44 & 24.69 & 68.73 & 61.00 & 21.57 & 55.32 & 38.86 \\
    \bottomrule
  \end{tabular}
}\vspace{-0.5em}
\caption{Per-category phrase localization accuracy(\%) of the NCE model and NCE+Distill model on the Flickr30K Entities dataset. Both models use Res101 CC as backbone. The NCE+Distillation model uses IRV2 OI as Detector$_{K}$.} \label{tab:flickr30k-per-category}\vspace{-1.5em}
\end{table*}
